Monotonic Properties of Completed Aggregates in Recursive Queries

The use of aggregates in recursion enables efficient and scalable support for a wide range of BigData algorithms, including those used in graph applications, KDD applications, and ML applications, which have proven difficult to be expressed and supported efficiently in BigData systems supporting Datalog or SQL. The problem with these languages and systems is that, to avoid the semantic and computational issues created by non-monotonic constructs in recursion, they only allow programs that are stratified with respect to negation and aggregates. Now, while this crippling restriction is well-justified for negation, it is frequently unjustified for aggregates, since (i) aggregates are often monotonic in the standard lattice of set-containment, (ii) the PreM property guarantees that programs with extrema in recursion are equivalent to stratified programs where extrema are used as post-constraints, and (iii) any program computing any aggregates on sets of facts of predictable cardinality tantamounts to stratified programs where the precomputation of the cardinality of the set is followed by a stratum where recursive rules only use monotonic constructs. With (i) and (ii) covered in previous papers, this paper focuses on (iii) using examples of great practical interest. For such examples, we provide a formal semantics that is conducive to efficient and scalable implementations via well-known techniques such as semi-naive fixpoint currently supported by most Datalog and SQL3 systems.

==> newrelated.tex <==
%This is the third  a last of the UCLA papers  presented at this 
%conference. These papers describe some surprising breakthroughs
 %achieved for Datalog, and also applicable
%to SQL and Prolog
%
%--They allow  efficient scalable support of classical polynomial time algorithms for BigData
%--The range of variety of these algorithms has been briefly illustrated in the previous section
%--The high level of performance and scalability obtained have been presented in  various 
%database conferences--the right environment because DB people   understand and  got
%rich on BigData parallelism and query optimization---although they might be a bit naive 
%when it comes to semantics.
%--Whereas here ICLP is indeed the right place to talk about semantics,  and my talk today
%focuses on that,
%
%But before will go into that let me remind you that the best student paper presented this morning
%that show that concepts such as Pre-mappability  that we intruduced to assure formal semantics 
%Have proven to be very conducive to improved performance ....
%%
%Outline
%
%Historical Background
%
%Pre-Mappability of Cosntraints
%
%Selected application examples
%
%Proving \prem--
%
%The simple cases,
%
%The complex cases requring formal tools
%
%Beyond Extrema
%
%-Conclusion
%Graph, ML, KDD





%!TEX root = pods17.tex
\inv\section{Related Work}
\label{sec:related}
% Several solutions, including  \cite{Kemp89propagatingconstraints,Srivastava92pushingconstraint}
% addressed  the problem of
% pushing comparison constraints into recursive rules, without exploring
%  relationships with the problems of supporting extrema and other
% aggregates into recursion.
The great opportunities and difficult problems created by aggregates in recursion
have been the topic of much research work in the past, for which
can only provide a high-level overview.   Many approaches
focused  on formal semantics that could accommodate
the non-monotonic nature of the aggregates. In particular \cite{DBLP:conf/vldb/MumickPR90}
discussed programs that are stratified w.r.t. aggregate operators
and proved that a perfect model exists for these programs, and \cite{DBLP:conf/slp/KempS91} defined extensions of the well-founded semantics to programs with aggregates.
% (such as the one of Example \ref{ex:ross_sagiv_example}).

The problem of  optimizing  programs with extrema 
by  early pruning non-relevant facts
was studied in \cite{DBLP:conf/pods/GangulyGZ91} and
\cite{DBLP:conf/vldb/SudarshanR91} under different optimization conditions, and
the notion of cost-monotonic  extrema aggregates was introduced in \cite{DBLP:journals/jcss/GangulyGZ95},
 using perfect models and well-founded
semantics. More recently, \cite{Furfaro:2002:PEA:599471.599473} devised an algorithm for pushing max and min constraints into recursion while preserving query equivalence under  specific monotonicity assumptions.
% whereas~\cite{DBLP:conf/pods/GrecoZG92} showed that
% to express greedy algorithms they require the  don't-care
%  non-determinism of the stable-model semantics
% provided by the choice construct.
%
% \cite{DBLP:conf/vldb/MumickPR90}\cite{DBLP:conf/slp/KempS91}
% \cite{DBLP:conf/pods/GangulyGZ91} and
%\cite{DBLP:conf/vldb/SudarshanR91}\cite{DBLP:journals/jcss/GangulyGZ95},  \cite{Furfaro:2002:PEA:599471.599473}  \cite{ross1992monotonic} \cite{van1993foundations}
%~\cite{DBLP:journals/jcss/RossS97}
% Those approaches provided effective optimization techniques for 
%  min and max aggregates in recursion, but did not
% consider %comparison constraints, 
% count and sum aggregates. The idea of relating comparison with extrema constraints is also used in~\cite{Liu:2012:CED:2398857.2384645} to optimize logical quantification.
A general approach to deal with all four aggregates
 was  proposed by \cite{ross1992monotonic} who advocated 
semantics based on specialized lattices, whereby each aggregate then defines a  monotonic
mapping in its special lattice---an approach that was not
 without practical limitations \cite{van1993foundations}.
%Meet and bag-monotonic are two special cases of Ross and Sagiv's approach~\cite{DBLP:journals/jcss/RossS97}.
% However,~\cite{van1993foundations} pointed out that automatically determining the correct lattices would be difficult in practice,
% and this was one of the causes that
% prevented the deployment of the monotonic-aggregate idea in query languages for the
% following twenty years.
A similar idea  was more recently proposed in \cite{Swift2010} and in  \cite{zhou2015planning} in the context of tabling in Prolog, using 3-valued well-founded model semantics.

Researchers working on Answer
Set Programming (ASP) have investigatd the benefits that aggregates offer in logic programs \cite{DBLP:journals/tplp/PelovDB07,DBLP:conf/lpnmr/PontelliSE04,DBLP:journals/tplp/SonP07}. 
%
%Tran Cao Son, Enrico Pontelli:
%A Constructive semantic characterization of aggregates in answer set programming. TPLP 7(3): 355-375 (2007)
%@article{DBLP:journals/tplp/SonP07,
%  author    = {Tran Cao Son and
%               Enrico Pontelli},
%  title     = {A Constructive semantic characterization of aggregates in answer set
%               programming},
%  journal   = {{TPLP}},
%  volume    = {7},
%  number    = {3},
%  pages     = {355--375},
%  year      = {2007},
%  url       = {https://doi.org/10.1017/S1471068406002936},
%  doi       = {10.1017/S1471068406002936},
%  timestamp = {Sat, 27 May 2017 14:23:06 +0200},
%  biburl    = {http://dblp.org/rec/bib/journals/tplp/SonP07},
%  bibsource = {dblp computer science bibliography, http://dblp.org}
%}
%
%Mario Alviano, Nicola Leone:
%On the Properties of GZ-Aggregates in Answer Set Programming. IJCAI 2016: 4105-4109
%
%@inproceedings{DBLP:conf/ijcai/AlvianoL16,
%  author    = {Mario Alviano and
%               Nicola Leone},
%  title     = {On the Properties of GZ-Aggregates in Answer Set Programming},
%  booktitle = {Proceedings of the Twenty-Fifth International Joint Conference on
%               Artificial Intelligence, {IJCAI} 2016, New York, NY, USA, 9-15 July
%               2016},
%  pages     = {4105--4109},
%  year      = {2016}
%
%
A new semantic analysis of the problem was proposed by \cite{DBLP:journals/tplp/GelfondZ14},  leading to the significant improvement discussed 
%
%Michael Gelfond, Yuanlin Zhang:
%Vicious Circle Principle and Logic Programs with Aggregates. TPLP 14(4-5): 587-601 (2014).
%@article{,
%  author    = {Michael Gelfond and
%               Yuanlin Zhang},
%  title     = {Vicious Circle Principle and Logic Programs with Aggregates},
%  journal   = {{TPLP}},
%  volume    = {14},
%  number    = {4-5},
%  pages     = {587--601},
%  year      = {2014}
%}
%
in \cite{DBLP:conf/ijcai/AlvianoL16}, and  various aggregate subclasses are
 identified for efficient   support in  the DLV system  \cite{DLV2}.

A renewed interest in Big Data analytics brought a revival of  Datalog with aggregates
in recursion. \cite{seo2013distributed,wang2015asynchronous}.
The treatment of extrema  presented in this paper extends  the monotonic count and sum
work of \cite{mazuran2013declarative} and provides the foundation for
the efficient and scalable systems discussed in \cite{bigdatalog},
\cite{DBLP:journals/vldb/YangSZ17},  and \cite{rasql}.








